Verifying Neural Networks Against Backdoor Attacks

Neural networks have achieved state-of-the-art performance in solving many problems, including many applications in safety/security-critical systems. Researchers also discovered multiple security issues associated with neural networks. One of them is backdoor attacks, i.e., a neural network may be embedded with a backdoor such that a target output is almost always generated in the presence of a trigger. Existing defense approaches mostly focus on detecting whether a neural network is 'backdoored' based on heuristics, e.g., activation patterns. To the best of our knowledge, the only line of work which certifies the absence of backdoor is based on randomized smoothing, which is known to significantly reduce neural network performance. In this work, we propose an approach to verify whether a given neural network is free of backdoor with a certain level of success rate. Our approach integrates statistical sampling as well as abstract interpretation. The experiment results show that our approach effectively verifies the absence of backdoor or generates backdoor triggers.

==> contents/appA.tex <==
\section{DeepPoly's Abstract Transformers}
\label{abs-rules}

Suppose we have constructed the abstract states of all the neurons up to layer $i$ and want to compute the abstract state of layer $i+1$. We first compute $ge^I_{i+1,j}$ and $le^I_{i+1,j}$ for each neuron $j$ in the layer $i+1$. If the layer $i+1$ is an activation function layer and the activation function is ReLU, we have the following.
\begin{align*}
    ge^I_{i+1,j} & = \begin{cases}
      \text{$0$} & \text{if $up^I_{i,j} \le -lw^I_{i,j}$} \\
      \text{$x^I_{i,j}$} & \text{otherwise}
    \end{cases}\\
    le^I_{i+1,j} & = \begin{cases}
    \text{$0$} & \text{if $up^I_{i,j} \le 0$} \\
    \text{$x^I_{i,j}$} & \text{if $lw^I_{i,j} \ge 0$} \\
    \text{$\dfrac{up^I_{i,j} \times (x^I_{i,j} - lw^I_{i,j})}{(up^I_{i,j} - lw^I_{i,j})}$} & \text{otherwise}
    \end{cases}
\end{align*}
If the activation function is the Sigmoid or Tanh function, we have the following. 
\begin{align*}
ge^I_{i+1,j} & = \begin{cases}
      \text{$\sigma(lw^I_{i,j})$} & \text{if $lw^I_{i,j} = up^I_{i,j}$}\\
      \text{$\sigma(lw^I_{i,j})+\lambda \times (x^I_{i,j} - lw^I_{i,j})$} & \text{if $lw^I_{i,j} > 0$}\\
      \text{$\sigma(lw^I_{i,j})+\lambda' \times (x^I_{i,j} - lw^I_{i,j})$} & \text{otherwise}
    \end{cases} \\
le^I_{i+1,j} & = \begin{cases}
      \text{$\sigma(up^I_{i,j})$} & \text{if $lw^I_{i,j} = up^I_{i,j}$}\\
      \text{$\sigma(up^I_{i,j})+\lambda \times (x^I_{i,j} - up^I_{i,j})$} & \text{if $up^I_{i,j} \le 0$}\\
      \text{$\sigma(up^I_{i,j})+\lambda' \times (x^I_{i,j} - up^I_{i,j})$} & \text{otherwise}
    \end{cases}
\end{align*}
where $\lambda = \dfrac{\sigma(up^I_{i,j}) - \sigma(lw^I_{i,j})}{up^I_{i,j} - lw^I_{i,j}}$; $\lambda' = \min(\sigma'(lw^I_{i,j}), \sigma'(up^I_{i,j}))$; $\sigma$ is the respective activation function; and $\sigma'$ is its first derivative. 

If the layer $i+1$ is an affine transformation layer, we have $ge^I_{i+1,j} = le^I_{i+1,j} = A_{i+1,j} \cdot x^I_{i,\cdot} + B_{i+1,j}$ where $A_{i+1,j}$ is the weight vector of neuron $j$ at layer $i+1$; $B_{i+1,j}$ is its bias; and $\cdot$ is the dot product. 

For the other 2 components $lw^I_{i+1,j}$ and $up^I_{i+1,j}$, if the layer $i+1$ is an activation function layer, we always have the upper bound $up^I_{i+1,j} = \sigma(up^I_{i,j})$ where $\sigma$ is the activation function. For the lower bound, if the activation function is Sigmoid or Tanh, we have $lw^I_{i+1,j} = \sigma(lw^I_{i,j})$. Otherwise, if the activation function is the ReLU function, we have the following.
\begin{align*}
    lw^I_{i+1,j} & = \begin{cases}
      \text{$0$} & \text{if $up^I_{i,j} \le -lw^I_{i,j}$} \\
      \text{$lw^I_{i,j}$} & \text{otherwise}
    \end{cases} 
\end{align*}

Finally, for the affine layer, back substitution is applied to compute the concrete lower bound and upper bound $lw^I_{i+1,j}$ and $up^I_{i+1,j}$. In particular, to compute the lower bound $lw^I_{i+1,j}$, we create a linear expression vector $ls^I_{i+1,j}$ with size $i+2$ and set $ls^I_{i+1,j}[i+1] = ge^I_{i+1,j} = A_{i+1,j} \cdot x^I_{i,\cdot} + B_{i+1,j}$. Afterwards, we compute $ls^I_{i+1,j}[s]$ for $0 \le s \le i$.
Note that at any step $s+1$, the value of $ls^I_{i+1,j}[s+1]$ can be expressed as a general linear expression of the form
$b + \sum_{h=0}^{n_s-1}{c^I_{s,h} \times x^I_{s,h}}$ where $b$ and each $c^I_{s,h}$ are constant values; and $x^I_{s,h}$ represents a particular variable at layer $s$. Thus, we have the following.
\begin{equation*}
\begin{split}
ls^I_{i+1,j}[s] = b & + \sum_{h=0}^{n_s-1}{\max(c^I_{s,h}, 0) \times ge^I_{s,h}} \\ & + \sum_{h=0}^{n_s-1}{\min(c^I_{s,h}, 0) \times le^I_{s,h}}
\end{split}
\end{equation*}

Intuitively, we substitute each variable in the expression by their corresponding $ge$ and $le$ expressions layer-by-layer. The process continues until $s=0$ and then we can set $lw^I_{i+1,j} = ls^I_{i+1,j}[0]$. Note that $ls^I_{i+1,j}[0]$ is always a constant. 

Similarly, to compute the upper bound $up^I_{i+1,j}$ for the variable $x^I_{i+1,j}$, we create another vector $us^I_{i+1,j}$ and set $us^I_{i+1,j}[i+1] = le^I_{i+1,j} = A_{i+1,j} \cdot x^I_{i,\cdot} + B_{i+1,j}$. Then we compute:
\begin{equation*}
\begin{split}
us^I_{i+1,j}[s] = b & + \sum_{h=0}^{n_s-1}{\min(c^I_{s,h}, 0) \times ge^I_{s,h}} \\ & + \sum_{h=0}^{n_s-1}{\max(c^I_{s,h}, 0) \times le^I_{s,h}}
\end{split}
\end{equation*}
for $0 \le s \le i$ before setting $up^I_{i+1,j} = us^I_{i+1,j}[0]$.

==> contents/appB.tex <==
\section{Optimization}

% \noindent \emph{Optimization} 
Note that at line 6 of Algorithm~\ref{alg:verify1}, for each constraint $\phi_I$, we perform a quick check to see if the constraint is satisfiable or not. If $\phi_I$ is UNSAT, we can ignore the remaining images and analyze the next trigger position, which allows us to speed up the process.
One naive approach is to call a solver on $\phi_I$, which would incur significant overhead since it could happen many times. To reduce the overhead, we propose a simple procedure to quickly check whether $\phi_I$ is UNSAT based solely on its abstract states at the output layer. That is, we check the satisfiability of the following constraint instead. 
$$\bigwedge_{0 \leq j < n_{l-1} \wedge j \neq t_s} up^I_{l-1,t_s} > lw^I_{l-1,j}$$
Recall that $up^I_{l-1,t_s}$ is the concrete upper bound of the neuron $t_s$ and $lw^I_{l-1,j}$ is the concrete lower bound of the  neuron $j$ at the output layer. Thus, intuitively, we check whether the concrete upper bound of the target label $t_s$ is larger than the concrete lower bound of every other label. If it is UNSAT, clearly it is impossible to have the target label as the classification result and thus the attack would fail on the image $I$.
We then only call the solver on $\phi_I$ if the above procedure does not return UNSAT.

Furthermore, it is easy to note that the loop in Algorithm~\ref{alg:verify1} can be parallelized straightforwardly, i.e., by using a separate process to verify against a different trigger position. Whenever a trigger is found by any of the processes, the whole algorithm is then interrupted. 
